On the Sample Complexity and Metastability of Heavy-tailed Policy Search in Continuous Control

Reinforcement learning is a framework for interactive decision-making with incentives sequentially revealed across time without a system dynamics model. Due to its scaling to continuous spaces, we focus on policy search where one iteratively improves a parameterized policy with stochastic policy gradient (PG) updates. In tabular Markov Decision Problems (MDPs), under persistent exploration and suitable parameterization, global optimality may be obtained. By contrast, in continuous space, the non-convexity poses a pathological challenge as evidenced by existing convergence results being mostly limited to stationarity or arbitrary local extrema. To close this gap, we step towards persistent exploration in continuous space through policy parameterizations defined by distributions of heavier tails defined by tail-index parameter alpha, which increases the likelihood of jumping in state space. Doing so invalidates smoothness conditions of the score function common to PG. Thus, we establish how the convergence rate to stationarity depends on the policy's tail index alpha, a Holder continuity parameter, integrability conditions, and an exploration tolerance parameter introduced here for the first time. Further, we characterize the dependence of the set of local maxima on the tail index through an exit and transition time analysis of a suitably defined Markov chain, identifying that policies associated with Levy Processes of a heavier tail converge to wider peaks. This phenomenon yields improved stability to perturbations in supervised learning, which we corroborate also manifests in improved performance of policy search, especially when myopic and farsighted incentives are misaligned.

==> Exittime.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Meta-Stability and Convergence to Wide Peaks}\label{subsec:exit_time}
We turn to characterizing the long-term behavior of Algorithm \ref{Algorithm2} in terms of its set of stationary points, specifically characterizing (i) the time it takes to escape a (possibly spurious) local extremum, and (ii) how the proportion of time spent at a local maxima depends on the width between its nearest local minima, which is determined by the policy's tail index. These results hinge upon a novel introduction into  reinforcement learning of metastability of dynamical systems under the influence of weak random perturbations \cite{tzen2018local}. Metastability refers to how transitions within the set of equilibria occur for the limit of a stochastic process. Such transitions happen even at a limit point may be interpreted as a form of persistent exploration for continuous space. 
%
Before discussing the main results of this subsection, we first present an additional condition we require on the score function.  
%
\begin{assumption}\label{Assump: disspitat}
	For some $m > 0$ and $b \geq 0$, $\nabla_{\bbtheta} \log \pi_{\bbtheta}(\cdot)$ is $(m,b,c)$-dissipative:
	\begin{align}
		c_{\alpha} \left< \bbtheta, \nabla_{\bbtheta} \log \pi_{\bbtheta}(\cdot) \right>  \geq    m \|\bbtheta\|^{1+c} -b, 
		\,  \forall \bbtheta \in \mathbb{R}^d.
	\end{align} 
\end{assumption}
%
%% Commenting +
We begin then by rewriting \eqref{eq:policy_gradient_iteration} in terms of the true policy gradient and the stochastic error $\hat{\nabla} J(\bbtheta_k)-\nabla {J}(\bbtheta_k)$, with the noise process hypothesized as an $\alpha$-tailed distribution.
%
% we can write \eqref{eq:policy_gradient_iteration5} as 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align} \label{eqn:SGD_L}
%
\bbtheta_{k+1} = \bbtheta_k + \eta \nabla_{\bbtheta}  J(\bbtheta_k) + \eta^{1/\alpha}  \eta^{\frac{\alpha-1}{\alpha}}  S_k\;,
%
\end{align}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $S_k \in \mathbb{R}^d$  is   $ \mathcal{S}\alpha \mathcal{S} $ distributed random vector.  Hereafter, we denote discrete-time process $\bbtheta_k$ by $\bbtheta^k$ with the time-index as a superscript to disambiguate between continuous and discrete stochastic processes. The update in \eqref{eqn:SGD_L} holds under a hypothesis that the stochastic errors associated with policy gradient steps are heavy-tailed, which has experimentally been observed under an extensive variety of contexts, such as Gaussian policies, in  \cite{garg2021proximal}. In Sec. \ref{sec:simulations}, we experimentally estimate the tail index associated with the gradient noise for different policies, and demonstrate that policies induce gradient noise with a tail index proportionate to that of its associated policy. 

%Hereafter, we denote discrete-time process $\bbtheta_k$ by $\bbtheta^k_t$ with the time-index as a superscript to disambiguate between continuous and discrete stochastic processes. 
 Under this representation, the continuous-time analogue of \eqref{eqn:SGD_L} (i.e., limit of $(\bbtheta_{k+1}-\bbtheta_k)/\eta$ as $\eta\rightarrow 0$) a Stochastic Differential Equation (SDE) driven by an $\alpha-$stable  L\'{e}vy process may be written as \cite{tzen2018local}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align}  \label{eqn:SGD_L1}
%
d\bbtheta_t^{\epsilon}  = \nabla_{\bbtheta} J(\bbtheta_t^{\epsilon}) dt +  \epsilon  d \bbL_t^{\alpha}\;,
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $\epsilon: = \eta^{\frac{\alpha-1}{\alpha}}$  is a coefficient that multiplies the jump process (analogous to the diffusion coefficient in Brownian motion), and  $\bbL_t$ denotes the multi-dimensional $\alpha$-stable L\'{e}vy motion in $\mathbb{R}^d$. 
%
%
Subsequently, we impose that the multi-dimensional L\'{e}vy motion $\bbL_t^\alpha$ admits a representation as a $\bbL_t^\alpha=\bbr L_t$ with $\bbr\in\mathbb{R}^d$ as a standard basis vector in $d$-dimensions, which determines the direction of the jump process, and $L_t$ is a scalar  $\alpha$-stable L\'{e}vy motion. This restriction is needed in order to tractably study the transient behavior of \eqref{eqn:SGD_L1} in terms of its exit time from regions of attraction \cite{imkeller2010first}, specifically, in applying Lemma \ref{lemma:bound}, as well as characterizing the proportion of time jumping between its limit points, to be discussed next. We note that such analyses for general $d$-dimensional  L\'{e}vy motion is an open problem in stochastic processes. 
%
Moreover, the validity of \eqref{eqn:SGD_L1} is only for the extent that tail index $\alpha \in (1,2]$ which we subsequently impose as a constraint on the range of $\alpha$.

With these details in place, we impose some additional structure (Assumption \ref{Assump:fun}) in Appendix \ref{subsec:exit_time_preliminaries} on the non-convex landscape of the objective $J(\bbtheta)$ in \eqref{eq:value_func}, namely, within the region of the objective's assumed finitely many local maxima, each one is separated by only a local minimum and no saddle points, as detailed in Appendix \ref{subsec:exit_time_preliminaries}. Conditions on the scalar L\'{e}vy process $L_t$ are also imposed in Assumption \ref{Assump_Levy} in Appendix \ref{subsec:exit_time_preliminaries}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Existing results on exit time and transition time are defined when the stochastic noise tends to zero, ie., $\epsilon \to 0$.
%Before discussing the main results, we first  summarize the assumptions  on the function, $J$ and stochastic noise, and define the terms associated with the meta-stability characteristics. \green{$F$ is undefined. We need to rewrite EVERYTHING in terms of maximizing $J(\bbtheta)$.} 
%\green{is the range for $\alpha\in (1,2)$ or $\alpha\in(0,2]$? This next assumption contradicts the above discussion.} 
%\blue{we may remove the below Assumption \ref{Assump_Levy} to Appendix}

%Next, we present  the assumptions on the L\'{e}vy process for $\alpha \in (1,2]$ in the scalar case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Defintions   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin by defining the common notions and assumptions used  for analyzing  meta-stability of the proposed setting. With the operating hypothesis that there are finitely many extrema of the objective, denote as   $\mathcal{G}_i \subset \mathbb{R}^d$  the neighborhood of the $i$-th local maximizer $\bar{\bbtheta}_i$  of radius $a+\xi$:
%
\begin{align} \label{eqn:_Gi}
%
\mathcal{G}_i:= \{ \mathbb{\bbtheta} \in \mathbb{R}^d: \| \bbtheta - \bar{\bbtheta}_i\| < a+ \xi \} \; , \qquad\partial \mathcal{G}_i:= \{ \mathbb{\bbtheta} \in \mathbb{R}^d: \| \bbtheta - \bar{\bbtheta}_i\| = a+ \xi \}
%
\end{align} 
%
where, $a, \, \xi >0$ are scalar radius parameters, and $\partial \mathcal{G}_i$ denotes the boundary of this neighborhood.
We assume  there exists atleast one set of  domains,  $\mathcal{G}_{i-1}$,  $\mathcal{G}_{i}$  and $\mathcal{G}_{i+1}$  such that $\mathcal{G}_{i-1}$,  $\mathcal{G}_{i}$  and $\mathcal{G}_{i+1}$ are connected,  $\partial \mathcal{G}_i \cap \partial \mathcal{G}_{j} \neq \emptyset, $ $j \in \{i-1, i+1\}$,
% \red{[AB:I think it should be $j \in \{i-1, i+1\}$?]},
  and  a  local minima, $s_j$   at the intersection of $\partial \mathcal{G}_i$ and $\partial \mathcal{G}_{j}$. This condition ensures that there is a direction from one local maxima to another. 

 For all   $(\bbtheta - \bar{\bbtheta}_i)$ at a distance $\bar{\delta}$ from $\partial \mathcal{G}_i$, we define  its distance to  $\partial \mathcal{G}_i$ along standard basis vector $\bbr\in\mathbb{R}^d$, where $\bbr$ is as in \eqref{eqn:SGD_L1} with $\bbL_t^\alpha=\bbr L_t$ in terms of the lines in $\mathbb{R}^d$ as $g_{i_{\bbtheta}}(t)= {\bbtheta} -\bar{\bbtheta}_i+t \cdot \bbr $ for $t \in \mathbb{R}$. Then, for all $\|\bbtheta-\bar{\bbtheta}_i\|	 < \bar{\delta}, \, \bar{\delta} \in (0, a+\xi)$,  the distance function to the boundary along $\bbr$ is defined as   
 %
\begin{align}\label{eqn:distm}
%
 d^+(\bbtheta):= \inf \{ t >0: g_{i_{\bbtheta}}(t) \in \partial \mathcal{G}_i \}\; ,\qquad % \\
%
  d^-(\bbtheta):= \sup \{ t <0: g_{i_{\bbtheta}}(t) \in \partial \mathcal{G}_i \},
%
\end{align}
%
where \eqref{eqn:distm}   define distance between   any point of interest and the  boundary of domain along  the  unit vector, $\bbr$, we have  $g_{i_{\bbtheta}}(t) \notin \mathcal{G}_i$ for $t \notin (d^-(\bbtheta), \, d^+(\bbtheta))$ for all $i$.  We say the point exits the domain $\mathcal{G}_i$ in the direction $\bbr$ when it enters the $\bar{\delta}$-tubes outside $\mathcal{G}_i$ defined by 
%
\begin{align} \label{eqn:omegatube}
%
 \Omega_i^+(\bar{\delta}):= \{\bbtheta \in \mathbb{R}^d: 	\|\left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right>\bbr -(\bbtheta- \bar{\bbtheta}_i)\| 	 <\bar{\delta},\, \left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right> > 0\} \cap \mathcal{G}_i^c.
%
\end{align}
%
  Analogously we define $\Omega_i^{-} (\bar{\delta})$ by changing to 
$\left<(\bbtheta- \bar{\bbtheta}_i), \bbr\right> < 0$.  Note that $\forall \bbtheta \in \Omega_i^+(\bar{\delta}), \|\bbtheta- \bar{\bbtheta}_i\| >a+\xi$.  
%
We note that  the term $\bbtheta- \bar{\bbtheta}_i$ is due to the fact that in \cite{imkeller2006first,imkeller2010first}, $\bb0$ is the stationary point of interest. Thus, we define $\bbtheta- \bar{\bbtheta}_i$ to shift towards the origin.

%
{\bf \noindent Exit Time and Transition Time.} Let us now  formally define the meta-stability characteristics, namely exit time and transition time  in  continuous time and then extend it  to the  the proposed heavy-tailed setting with  the assumption that  \eqref{eqn:SGD_L1}  and \eqref{eqn:SGD_L} are initialized at ${\bbtheta_0}$  inside $\mathcal{G}_i$.
 
 %
\begin{definition}\label{def:exit_time}
%
({\bf Exit time  from $\mathcal{G}_i$}) The time required  for the continuous-time process \eqref{eqn:SGD_L1} and discrete-time process \eqref{eqn:SGD_L}, respectively, to exit  $\mathcal{G}_i$ along $ + \bbr$  is defined by 
%Let  $\bbtheta_t =\bbtheta_k, \, t=k\eta=0$ (both discrete and continuous processes are initialized with $\bbtheta_0$) and the time required  to exit the basin $[0, a+\xi]$ by the process \eqref{eqn:SGD_L1} is defined by 
%
\begin{align}\label{exit_contins}
%
%& \hat{\tau}_{\xi,a} (\epsilon) \triangleq \inf \{ t \geq 0:  \| \bbtheta_t -\bar{\bbtheta}\| \notin [0, a + \xi]  \}, \\
%& \green{
\hat{\tau}_{\xi,a}(\epsilon) \triangleq \inf \{ t \geq 0:  \bbtheta_t^{\epsilon} \in  \Omega_i^+(\bar{\delta})   \}, \qquad
%
%\end{align}
%
%and the time at which the discrete time process \eqref{eqn:SGD_L} exits $\mathcal{G}_i$ is given by 
%
%\begin{align} \label{eqn:taudisccrt}
%
%& \bar{\tau}_{\xi,a} (\epsilon) \triangleq \inf \{ K \in \mathbb{N} :  \| \bbtheta^k -\bar{\bbtheta}\| \notin [0, a + \xi]  \} \\
%& \green{
\bar{\tau}_{\xi,a}(\epsilon) \triangleq \inf \{ K \in \mathbb{N} :   \bbtheta^K  \in  \Omega_i^+(\bar{\delta})  \}.
%
\end{align}
%
\end{definition}
%
Here, $a$ and $\xi$ denote scalar radius parameters (cf. \eqref{eqn:_Gi}). We underscore that $\bar{\tau}(\cdot)$ represents the exit time of discrete-time process $\bbtheta^k$, whereas $\hat{\tau} (\cdot) $ denotes that of continuous-time stochastic process $\bbtheta_t^{\epsilon}$. 
[\red{AB:
%what does $\xi$ denotes in the above definitions?
 little confusion about the superscript $k$ with $\bbtheta$ here?}]

\begin{definition}\label{def:transition_time}
%
({\bf Transition time from $\mathcal{G}_i$ to $\mathcal{G}_j$})
%
%\paragraph{Transition time from $\mathcal{G}_i$ to $\mathcal{G}_j$:} 
 Under the existence of a unit vector $\bbr$ along the direction connecting the domains $\mathcal{G}_i$ and $\mathcal{G}_{i+1}$ between two distinct local maxima, we define the transition time  from a neighborhood of one local maxima to another, i.e., from $\mathcal{G}_i$ to $\mathcal{G}_j, \, i\neq j$ in respective continuous-time [cf. \eqref{eqn:SGD_L1}] and discrete-time \eqref{eqn:SGD_L} 
%
\begin{align}\label{eq:transition_time}
%
\hat{T}_{i} (\epsilon) =  \inf \{   t>0: \bbtheta_{t}^{\epsilon}  \in \cup_{i \neq j} \mathcal{G}_j  \}\;,\qquad
%
%\end{align}
%
%and the time at which the discrete time process \eqref{eqn:SGD_L} transitions away from $\mathcal{G}_i$ is given by 
%
%\begin{align}
%
\bar{T}_{i} (\epsilon) = \inf\{   K \in \mathbb{N}: \bbtheta^{K}   \in \cup_{i \neq j} \mathcal{G}_j  \}\;. 
%
\end{align}
%
\end{definition}
%\red{AB: $\inf$ outside the curly bracket?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%T  H  E  O  R  E  M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The following theorems present the first exit time and transition time probabilities of  the proposed heavy-tailed policy gradient setting, \eqref{eq:policy_gradient_iteration00} when initialized within  $\mathcal{G}_i \subset \mathbb{R}^d$ such that \eqref{eqn:_Gi} holds.
%
%\green{There are several issues here:
%
%\begin{enumerate}
%%
%\item $\mathcal{G}$ seems undefined. How is this different from $\mathbb{R}^d$? I believe we are permitting the feasible set of $\bbtheta$ to be unbounded within $\mathbb{R}^d$, correct?
%%
%\item $ \bar{\tau}_{0,a} (\epsilon) >K$ needs to be defined here, as does the set of local minima/maxima, and all the quantities in Theorem \ref{Theorem:Exit_time}. For instance, the definition of $M,d^+,K$ are missing rigorous/specific definitions. Some of that is defined at the beginning of Appendix \ref{Proof:exittime}, but it needs to be here instead/also.
%%
%\item The statement formalizing the transition probabilities of the limiting process is missing from this section (specifically, the contents of Appendix \ref{apx_transition_time}.
%%
%\end{enumerate}
%%
%}
\begin{theorem}(Exit Time Dependence on Tail Index) \label{Theorem:Exit_time}
%
%
Under Assumptions \ref{Assum:Q0}- \ref{assmp:domaing}, if the value function $J$  is initialized near a local maxima $\bar{\bbtheta}_i$, then the policy gradient update in \eqref{eq:policy_gradient_iteration00} under a heavy-tailed parameterization with tail index $\alpha$ associated with its induced stochastic error \eqref{eqn:SGD_L}, exits from the neighborhood  of $\bar{\bbtheta}_i$  at an exit time  $\bar{\tau}_{0,a}$  
with a positive probability given by 
%
\begin{align}\label{eq:exit_time_theorem}
%
\!\!\! \mathcal{P}^{\bbtheta_0} \!\left(  \bar{\tau}_{0,a} (\epsilon) >\!K\right) 
 %
  &\leq \frac{2}{\epsilon^{\rho \alpha}} \epsilon^{\alpha} (d^+)^{-\alpha}   \!+\!   \mathcal{O} \!\!\left( \!\! \left(\frac{d}{k_1^{1/\alpha}} K \eta\right)^{\beta}  \!\!\!+\! \left(\!\!-d^{1+\frac{\alpha}{2}} \exp{(\alpha M_J\eta)}\epsilon^{\alpha}\!\!\left(\frac{\xi}{3}\right)^{\!\!-\alpha}\right)^{\!\!\!K} \right)\!
 %
\end{align}
%
%\red{AB: what is $k_1$ here?}
where, $\bbtheta_0$ is the point of initialization, the neighborhood of   local maxima  is denoted by $\mathcal{G}$, $d^+$  denotes distance  between $\bbtheta_0$ and the boundary of $\mathcal{G}$,  $\rho$ is a positive constant such that $\rho \in (0,1)$,  $\alpha$  the  tail-index,  $d$ is the dimension of $\bbtheta$. Moreover, the H\"{o}lder continuity constant satisfies $\beta \in (0,\alpha-1)$, $\delta >0$,  $\xi>0$,  $\eta$ is the step-size, $k_1$ is a function of stepsize $\eta$, $k_1: = 1/\eta^{\alpha-1}$, and $\epsilon$ is the coefficient multiplying the jump process. 
\end{theorem}

\red{AB: may be one way to interpret these results is first we fix large $K$, and then we interpret how the probability of exit time being grater that $K$ is controlled by the parameter $\alpha$. We need to provide this intuition, it is not very clear by just looking at the expressions in \eqref{eq:exit_time_theorem}. }
\begin{proof}
The proof is provided in Appendix \ref{Proof:exittime}.
\end{proof}



\begin{theorem} (Transition Time Dependence on Tail Index)\label{theorem: transitiontym}
Suppose Assumptions \ref{Assum:Q0}- \ref{assmp:domaing} hold and the value function $J$  is initialized near a local maxima $\bar{\bbtheta}_i$. Then in the limit $\epsilon \to 0$,  the policy gradient update in \eqref{eq:policy_gradient_iteration00} under a heavy-tailed parameterization with tail index $\alpha$ associated with its induced stochastic error \eqref{eqn:SGD_L}, transitions from $\mathcal{G}_i$ to the boundary of $(i+1)$-th local maxima with a probability, $\mathcal{P}^{\bbtheta_0}( \bbtheta^{k} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) $  lower bounded by the following function of the tail index $\alpha$:
%
 \begin{align} \label{eqn:thm4}
%
\lim_{\epsilon \to 0} \mathcal{P}^{\bbtheta_0}( \bbtheta_{k\eta} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) \geq \frac{d_{ij}^{-\alpha}}{((d_{ij}^+)^{-\alpha} + (-d_{ij}^-)^{-\alpha}}  - \delta,
%
\end{align}
where $\delta >0$ and distance function:
%
\begin{align}\label{eqn:dista}
%
\! \!\!d_{ij}^+(\bbtheta)\!:=\! \inf \{ t\! >\!0\!:\! g_{{i}_{\bbtheta}}(t) \!\in\! \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1} \!\}, \ %  \\
  d_{ij}^-(\bbtheta)\!:=\! \sup \{ t \!<\!0\!:\! g_{{i}_{\bbtheta}}(t) \!\in\! \Omega_i^- (\bar{\delta}) \cap \partial \mathcal{G}_{i+1} \!\}.\!\!
%
\end{align}
\end{theorem}
% \textcolor{green}{need to more rigorously define $\lambda_k^\alpha$ and $N$. Also, what is $\xi$? This is a positive constant but why is it defined? To introduce slack in a neighborhood of $a$? Moreover, $p_i^{-}$ seems unused in \eqref{eq:exit_time_theorem}. Why is it defined?}

%$U_R$, $\gamma$ are the parameters of proposed RL setting, positive constants, $C, \, C_1\, C_2$,   are functions of dissipativity constants of score function, 
%\begin{align}
%\mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq &  \exp{\left(-K\eta \epsilon^{\alpha} \frac{1}{a^{\alpha}\alpha}(1+C\epsilon^{\delta})\right)} (1+ C \epsilon^{\delta}) +  \exp{(M\eta)}  M \eta  \frac{   C_1  \left( 1 + C_2 \left(\frac{U_R}{(1-\gamma)^2}  (m +b)/2   + C \frac{d}{k_1^{1/\alpha}}   \right)K\eta \right)^{\beta}}{\xi/3}     \nonumber \\
% & +  1- \left(1-C_{\alpha}d^{1+\frac{\alpha}{2}}\eta \exp{(\alpha M\eta)}\epsilon^{\alpha}\left(\frac{\xi}{3}\right)^{-\alpha}\right)^{K} +\delta,
%\end{align}
\begin{proof}
The proof is provided in Appendix \ref{sec:proofthm4}.
\end{proof}

Observe that the transition time probabilities here is a function of  distance between the local extrema and tail-index, $\alpha$, similar to the  results for single dimensional case \cite{imkeller2006first}.   \blue{It is interesting to note that with  small noise limit ($\epsilon \to 0$) of  \eqref{eq:exit_time_theorem},   the probability of escape from a given neighborhood  depends  on the  distance of $\bbtheta_0$ from the boundary $\partial \mathcal{G}$ and tail-index, $\alpha$. Further  the probability of escape from local extrema is inversely proportional to the width of the boundary.  Therefore, the proposed heavy-tailed setting prefers wide minima and  its escape probability increases  with  heavier  tail indices. 
Corresponding expressions for vanilla policy gradient of \eqref{SGD:G2} wherein the stochastic error is a Brownian noise (cf.  \eqref{SGD:G3} is summarized in Table \ref{table_1}. In contrast to proposed heavy-tailed setting wherein transition probability is a function of width of the a neighborhoods, expression for  \eqref{SGD:G3}  depends on the   function value at the extremas. In other words, in the small noise limit Brownian motion takes  exponential time to transit to the immediate local extrema \cite{bouchet2016generalisation}. }
\green{we need a comment about how the transition time only depends on the width of the peak, but not the height, in contrast to classical (fat-tailed) central limit theorem associated with Gaussians. Classical result like \cite{raginsky2017non} should also have some exponential dependence on the parameter dimension that we are alleviating, right?}


\red{[AB: One most important part which is missing from the discussion here I feel is about the interpretation of the mathematical equations in the statement of both the Theorem. For instance, We need to state something like how this $\alpha$ or $\beta$ is actually controlling the exit/transition time in words. Another important factor here could be related to the association of these results in the RL   settings. What are the new interesting dependencies we get which are specific   to the RL settings. I am just writing down my thoughts so that we could discuss tomorrow. We may need to emphasize more in words about the major take away message of this subsection " local extrema with wider peaks" which we claimed in the end of previous subsection.  ]}
%\begin{center}
%	\begin{tabularx}{01\textwidth} { 
%  | >{\centering\arraybackslash}X 
%  | >{\raggedright\arraybackslash}X | >{\raggedright\arraybackslash}X|}
%		\hline
%Algorithm  & Exit time & Transition time   \\
%		\hline
%	HPG &  $ \mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq \frac{2}{\epsilon^{\rho \alpha}} \epsilon^{\alpha} (d^+)^{-\alpha}  + \mathcal{O} \left( \frac{d}{k_1^{1/\alpha}} K \eta\right)^{\beta}  + \mathcal{O} \left(d^{1+\frac{\alpha}{2}} \epsilon^{\alpha}\left(\frac{\xi}{3}\right)^{-\alpha}\right)^{K} $  &  $\lim_{\epsilon \to 0} \mathcal{P}^{\bbtheta_0}( \bbtheta_{k\eta} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) \geq \frac{d_{ij}^{-\alpha}}{((d_{ij}^+)^{-\alpha} + (-d_{ij}^-)^{-\alpha}}  - \delta$\\
%  		\hline
%  	Vanilla PG &  $\mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq $ \blue{Need to find this expression: immediate step} &  \\
%
%		\hline
%	\end{tabularx}
%	%\caption{First Exit time of Algorithms}
%\end{center}
%\blue{Note: Once we finalize the analysis for the above Theorem we can directly invoke results for Vanilla PG with constant variance. We need to the exit time for Brownian in  $\mathbb{R}^d$ from the literature and relate it to discrete process. Note that the Theorems from Mert et al. is for one dimensional case. Below, I briefly summarize the corresponding expression of SDE for Brownian case. This would be our starting point and we follow same steps as followed for the above Theorem except that L\'{e}vy process will now be replaced by Brownian. Also, lot of parts will be simplified as we just need Lipschitz continuity. }\green{please fill in this table as it pertains to usual policy parameterizations (e.g., Gaussian)}
{Note that  for vanilla policy gradients (Example \ref{eg:gaussian_fixed_var}), the stochastic error reduces to Brownian noise and  we have
\begin{align}\label{SGD:G2}
\bbtheta^{k+1} = \bbtheta^k +\eta \nabla J(\bbtheta^k) + \sqrt{\eta} \sqrt{\eta \sigma^2} \bbZ_k,
\end{align}
where, $\bbZ_k$ denotes the standard normal vector in $\mathbb{R}^d$ and the continuous-time analogue of the above process for $\epsilon: \sqrt{\eta \sigma^2}  \to 0$   takes the form
\begin{align}\label{SGD:G3}
d\bbtheta_t^{\epsilon}  = \nabla J(\bbtheta_t^{\epsilon}) dt + {\epsilon} d\bbB_t,
\end{align}
where, $\bbB_t$ is the standard Brownian motion. 

\red{AB: May be we could completely remove the vanilla PG case from the main body of the paper?}}

==> Exittime_amrit.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Meta-Stability and Convergence to Wide Peaks}\label{subsec:exit_time}
We turn to characterizing the long-term behavior of Algorithm \ref{Algorithm2} in terms of its set of stationary points, specifically characterizing (i) the time it takes to escape a (possibly spurious) local extremum, and (ii) how the proportion of time spent at a local maxima depends on the width between its nearest local minima, which is determined by the policy's tail index. These results hinge upon a novel introduction into  reinforcement learning of metastability of dynamical systems under the influence of weak random perturbations \cite{tzen2018local}.
% Metastability refers to how transitions within the set of equilibria occur for the limit of a stochastic process. Such transitions happen even at a limit point may be interpreted as a form of persistent exploration for continuous space. 
%
Before discussing the main results of this subsection, we first present an additional condition we require on the score function.  
%
\begin{assumption}\label{Assump: disspitat}
	For some $m > 0$ and $b \geq 0$, $\nabla_{\bbtheta} \log \pi_{\bbtheta}(\cdot)$ is $(m,b,c)$-dissipative, which implies that
	%\begin{align}
	$	c_{\alpha} \left< \bbtheta, \nabla_{\bbtheta} \log \pi_{\bbtheta}(\cdot) \right>  \geq    m \|\bbtheta\|^{1+c} -b$, for all $\bbtheta \in \mathbb{R}^d$.
%	\end{align} 
\end{assumption}
%
%% Commenting +
We begin then by rewriting \eqref{eq:policy_gradient_iteration} in terms of the true policy gradient and the stochastic error $\hat{\nabla} J(\bbtheta_k)-\nabla {J}(\bbtheta_k)$, with the noise process hypothesized as an $\alpha$-tailed distribution, given by 
%
% we can write \eqref{eq:policy_gradient_iteration5} as 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align} \label{eqn:SGD_L}
%
\bbtheta_{k+1} = \bbtheta_k + \eta \nabla_{\bbtheta}  J(\bbtheta_k) + \eta^{1/\alpha}  \eta^{\frac{\alpha-1}{\alpha}}  S_k\;,
%
\end{align}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $S_k \in \mathbb{R}^d$  is   $ \mathcal{S}\alpha \mathcal{S} $ distributed random vector.  Hereafter, we denote discrete-time process $\bbtheta_k$ by $\bbtheta^k$ with the time-index as a superscript to disambiguate between continuous and discrete stochastic processes. The update in \eqref{eqn:SGD_L} holds under a hypothesis that the stochastic errors associated with policy gradient steps are heavy-tailed, which has experimentally been observed under an extensive variety of contexts, such as Gaussian policies, in  \cite{garg2021proximal}. In Sec. \ref{sec:simulations}, we experimentally estimate the tail index associated with the gradient noise for different policies, and demonstrate that policies induce gradient noise with a tail index proportionate to that of its associated policy. 
%
\begin{table}\label{table_1}
	\centering
	\resizebox{0.6\linewidth}{!}{
		\begin{tabular}{|p{1.3cm}|p{2.2cm}|p{3cm}|p{3.2cm}|} 
			%	{ | >{}X| >{}X| >{}X| >{}X| }
			\hline
			Algorithm & Iter. complexity & Exit time (cf. \eqref{exit_contins}) & Trans. time (cf. \eqref{eq:transition_time})\\
			\hline
			PG   & $\mathcal{O}\left({1}/{\kappa^{2}}\right)$  &  $\mathcal{O} \left(   e^{-2 J(a)/\epsilon^2} \right) $  %\cite{imkeller2006first,nguyen2019first}
			&   $  \mathcal{O} \left( e^{2 (J(\bar{\bbtheta}_i)-J(\bar{\bbtheta}_i ))/\epsilon^{2}}\right) $  
			%\cite{bouchet2016generalisation})
			\\
			\hline
			HPG& $\mathcal{O}\left({1}/{\kappa^{1+\frac{1}{\beta}}}\right)$  & $\mathcal{O} \left(  \frac{\alpha}{2} \frac{a^{\alpha}}{\epsilon^{\alpha}} \right) $  & $ \mathcal{O} \left( 1/\epsilon^{\alpha}\right) $   \\
			\hline
	\end{tabular}
}
	\caption{\scriptsize Summary of iteration complexity, exit  time, and transition time results  for vanilla PG and heavy-tailed PG algorithms ( $\epsilon$:  coefficient that multiplies the jump process). \vspace{-6mm}}
\end{table}
%
%Hereafter, we denote discrete-time process $\bbtheta_k$ by $\bbtheta^k_t$ with the time-index as a superscript to disambiguate between continuous and discrete stochastic processes. 
 Under this representation in \eqref{eqn:SGD_L}, the continuous-time analogue of \eqref{eqn:SGD_L} (i.e., limit of $(\bbtheta_{k+1}-\bbtheta_k)/\eta$ as $\eta\rightarrow 0$) can be written as a Stochastic Differential Equation (SDE) driven by an $\alpha-$stable  L\'{e}vy process as \cite{tzen2018local}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align}  \label{eqn:SGD_L1}
%
d\bbtheta_t^{\epsilon}  = \nabla_{\bbtheta} J(\bbtheta_t^{\epsilon}) dt +  \epsilon  d \bbL_t^{\alpha}\;,
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $\epsilon: = \eta^{\frac{\alpha-1}{\alpha}}$  is a coefficient that multiplies the jump process (analogous to the diffusion coefficient in Brownian motion), and  $\bbL_t^\alpha$ denotes the multi-dimensional $\alpha$-stable L\'{e}vy motion in $\mathbb{R}^d$. 
%
%
%Subsequently, we impose that the multi-dimensional L\'{e}vy motion $\bbL_t^\alpha$ admits a representation as a $\bbL_t^\alpha=\bbr L_t$ with $\bbr\in\mathbb{R}^d$ as a standard basis vector in $d$-dimensions, which determines the direction of the jump process, and $L_t$ is a scalar  $\alpha$-stable L\'{e}vy motion. This restriction is needed in order to tractably study the transient behavior of \eqref{eqn:SGD_L1} in terms of its exit time from regions of attraction \cite{imkeller2010first}, specifically, in applying Lemma \ref{lemma:bound}, as well as characterizing the proportion of time jumping between its limit points, to be discussed next. We note that such analyses for general $d$-dimensional  L\'{e}vy motion is an open problem in stochastic processes. 
%
%Moreover, the validity of \eqref{eqn:SGD_L1} is only for the extent that tail index $\alpha \in (1,2]$ which we subsequently impose as a constraint on the range of $\alpha$.
%
With these details in place, we impose some additional structure (Assumption \ref{Assump:fun}) in Appendix \ref{subsec:exit_time_preliminaries} on the non-convex landscape of the objective $J(\bbtheta)$ in \eqref{eq:value_func}, namely, within the region of the objective's assumed finitely many local maxima, each one is separated by only a local minimum and no saddle points, as detailed in Appendix \ref{subsec:exit_time_preliminaries}.
% Conditions on the scalar L\'{e}vy process $L_t$ are also imposed in Assumption \ref{Assump_Levy} in Appendix \ref{subsec:exit_time_preliminaries}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Existing results on exit time and transition time are defined when the stochastic noise tends to zero, ie., $\epsilon \to 0$.
%Before discussing the main results, we first  summarize the assumptions  on the function, $J$ and stochastic noise, and define the terms associated with the meta-stability characteristics. \green{$F$ is undefined. We need to rewrite EVERYTHING in terms of maximizing $J(\bbtheta)$.} 
%\green{is the range for $\alpha\in (1,2)$ or $\alpha\in(0,2]$? This next assumption contradicts the above discussion.} 
%\blue{we may remove the below Assumption \ref{Assump_Levy} to Appendix}
%
%Next, we present  the assumptions on the L\'{e}vy process for $\alpha \in (1,2]$ in the scalar case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Defintions   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
 With the operating hypothesis that there are finitely many extrema of the objective, denote as   $\mathcal{G}_i \subset \mathbb{R}^d$  the neighborhood of the $i$-th local maximizer $\bar{\bbtheta}_i$  of radius $a+\xi$:
%
\begin{align} \label{eqn:_Gi}
%
\mathcal{G}_i:= \{ \mathbb{\bbtheta} \in \mathbb{R}^d: \| \bbtheta - \bar{\bbtheta}_i\| < a+ \xi \} \; , \qquad\partial \mathcal{G}_i:= \{ \mathbb{\bbtheta} \in \mathbb{R}^d: \| \bbtheta - \bar{\bbtheta}_i\| = a+ \xi \}
%
\end{align} 
%
where, $a, \, \xi >0$ are scalar radius parameters, and $\partial \mathcal{G}_i$ denotes the boundary of this neighborhood.
%We assume  there exists atleast one set of  domains,  $\mathcal{G}_{i-1}$,  $\mathcal{G}_{i}$  and $\mathcal{G}_{i+1}$  such that $\mathcal{G}_{i-1}$,  $\mathcal{G}_{i}$  and $\mathcal{G}_{i+1}$ are connected,  $\partial \mathcal{G}_i \cap \partial \mathcal{G}_{j} \neq \emptyset, $ $j \in \{i-1, i+1\}$,
% \red{[AB:I think it should be $j \in \{i-1, i+1\}$?]},
%  and  a  local minima, $s_j$   at the intersection of $\partial \mathcal{G}_i$ and $\partial \mathcal{G}_{j}$. This condition ensures that there is a direction from one local maxima to another. 
%

%
%
% For all   $(\bbtheta - \bar{\bbtheta}_i)$ at a distance $\bar{\delta}$ from $\partial \mathcal{G}_i$, we define  its distance to  $\partial \mathcal{G}_i$ along standard basis vector $\bbr\in\mathbb{R}^d$, where $\bbr$ is as in \eqref{eqn:SGD_L1} with $\bbL_t^\alpha=\bbr L_t$ in terms of the lines in $\mathbb{R}^d$ as $g_{i_{\bbtheta}}(t)= {\bbtheta} -\bar{\bbtheta}_i+t \cdot \bbr $ for $t \in \mathbb{R}$. Then, for all $\|\bbtheta-\bar{\bbtheta}_i\|	 < \bar{\delta}, \, \bar{\delta} \in (0, a+\xi)$,  the distance function to the boundary along $\bbr$ is defined as   
% %
%\begin{align}\label{eqn:distm}
%%
% d^+(\bbtheta):= \inf \{ t >0: g_{i_{\bbtheta}}(t) \in \partial \mathcal{G}_i \}\; ,\qquad % \\
%%
%  d^-(\bbtheta):= \sup \{ t <0: g_{i_{\bbtheta}}(t) \in \partial \mathcal{G}_i \},
%%
%\end{align}
%%
%where \eqref{eqn:distm}   define distance between   any point of interest and the  boundary of domain along  the  unit vector, $\bbr$, we have  $g_{i_{\bbtheta}}(t) \notin \mathcal{G}_i$ for $t \notin (d^-(\bbtheta), \, d^+(\bbtheta))$ for all $i$.  We say the point exits the domain $\mathcal{G}_i$ in the direction $\bbr$ when it enters the $\bar{\delta}$-tubes outside $\mathcal{G}_i$ defined by 
%%
%\begin{align} \label{eqn:omegatube}
%%
% \Omega_i^+(\bar{\delta}):= \{\bbtheta \in \mathbb{R}^d: 	\|\left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right>\bbr -(\bbtheta- \bar{\bbtheta}_i)\| 	 <\bar{\delta},\, \left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right> > 0\} \cap \mathcal{G}_i^c.
%%
%\end{align}
%%
%  Analogously we define $\Omega_i^{-} (\bar{\delta})$ by changing to 
%$\left<(\bbtheta- \bar{\bbtheta}_i), \bbr\right> < 0$.  Note that $\forall \bbtheta \in \Omega_i^+(\bar{\delta}), \|\bbtheta- \bar{\bbtheta}_i\| >a+\xi$.  
%%
%We note that  the term $\bbtheta- \bar{\bbtheta}_i$ is due to the fact that in \cite{imkeller2006first,imkeller2010first}, $\bb0$ is the stationary point of interest. Thus, we define $\bbtheta- \bar{\bbtheta}_i$ to shift towards the origin.

%
{\bf \noindent Exit Time and Transition Time.} Let us now  formally define the meta-stability characteristics, namely exit time and transition time  in  continuous time and then extend it  to the  the proposed heavy-tailed setting with  the assumption that  \eqref{eqn:SGD_L1}  and \eqref{eqn:SGD_L} are initialized at ${\bbtheta_0}$  inside $\mathcal{G}_i$.
 
 %
\begin{definition}\label{def:exit_time0}
%
({\bf Exit time  from $\mathcal{G}_i$}) The time required  for the continuous-time process \eqref{eqn:SGD_L1} and discrete-time process \eqref{eqn:SGD_L}, respectively, to exit  $\mathcal{G}_i$ along standard basis vector $\bbr\in\mathbb{R}^d$  is defined by 
%Let  $\bbtheta_t =\bbtheta_k, \, t=k\eta=0$ (both discrete and continuous processes are initialized with $\bbtheta_0$) and the time required  to exit the basin $[0, a+\xi]$ by the process \eqref{eqn:SGD_L1} is defined by 
%
%\begin{align}\label{exit_contins}
%
%& \hat{\tau}_{\xi,a} (\epsilon) \triangleq \inf \{ t \geq 0:  \| \bbtheta_t -\bar{\bbtheta}\| \notin [0, a + \xi]  \}, \\
%& \green{
$\hat{\tau}_{\xi,a}(\epsilon) \triangleq \inf \{ t \geq 0:  \bbtheta_t^{\epsilon} \in  \Omega_i^+(\bar{\delta})   \}, \qquad
%
%\end{align}
%
%and the time at which the discrete time process \eqref{eqn:SGD_L} exits $\mathcal{G}_i$ is given by 
%
%\begin{align} \label{eqn:taudisccrt}
%
%& \bar{\tau}_{\xi,a} (\epsilon) \triangleq \inf \{ K \in \mathbb{N} :  \| \bbtheta^k -\bar{\bbtheta}\| \notin [0, a + \xi]  \} \\
%& \green{
\bar{\tau}_{\xi,a}(\epsilon) \triangleq \inf \{ K \in \mathbb{N} :   \bbtheta^K  \in  \Omega_i^+(\bar{\delta})  \}.
%
%\end{align}
%
\end{definition}
%
Here, $a$ and $\xi$ denote scalar radius parameters (cf. \eqref{eqn:_Gi}). In \eqref{exit_contins},  $\Omega_i^+(\bar{\delta})$ denote the $\bar\delta\in(0, a+\xi)$ tubes outside $\mathcal{G}_i$ defined by 
%
%
\begin{align} \label{eqn:omegatube}
	%
	\Omega_i^+(\bar{\delta}):= \{\bbtheta \in \mathbb{R}^d: 	\|\left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right>\bbr -(\bbtheta- \bar{\bbtheta}_i)\| 	 <\bar{\delta},\, \left<(\bbtheta- \bar{\bbtheta}_i), \bbr \right> > 0\} \cap \mathcal{G}_i^c.
	%
\end{align}
%
We underscore that $\bar{\tau}(\cdot)$ represents the exit time of discrete-time process $\bbtheta^k$, whereas $\hat{\tau} (\cdot) $ denotes that of continuous-time stochastic process $\bbtheta_t^{\epsilon}$. 

\begin{definition}\label{def:transition_time}
%
({\bf Transition time from $\mathcal{G}_i$ to $\mathcal{G}_j$})
%
%\paragraph{Transition time from $\mathcal{G}_i$ to $\mathcal{G}_j$:} 
 Under the existence of a unit vector $\bbr$ along the direction connecting the domains $\mathcal{G}_i$ and $\mathcal{G}_{i+1}$ between two distinct local maxima, we define the transition time  from a neighborhood of one local maxima to another, i.e., from $\mathcal{G}_i$ to $\mathcal{G}_j, \, i\neq j$ in respective continuous-time [cf. \eqref{eqn:SGD_L1}] and discrete-time \eqref{eqn:SGD_L} 
%
\begin{align}\label{eq:transition_time}
%
\hat{T}_{i} (\epsilon) =  \inf \{   t>0: \bbtheta_{t}^{\epsilon}  \in \cup_{i \neq j} \mathcal{G}_j  \}\;,\qquad
%
%\end{align}
%
%and the time at which the discrete time process \eqref{eqn:SGD_L} transitions away from $\mathcal{G}_i$ is given by 
%
%\begin{align}
%
\bar{T}_{i} (\epsilon) = \inf\{   K \in \mathbb{N}: \bbtheta^{K}   \in \cup_{i \neq j} \mathcal{G}_j  \}\;. 
%
\end{align}
%
\end{definition}
%\red{AB: $\inf$ outside the curly bracket?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%T  H  E  O  R  E  M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The following theorems present the first exit time and transition time probabilities of  the proposed heavy-tailed policy gradient setting, \eqref{eq:policy_gradient_iteration00} when initialized within  $\mathcal{G}_i \subset \mathbb{R}^d$ such that \eqref{eqn:_Gi} holds.
%
%\green{There are several issues here:
%
%\begin{enumerate}
%%
%\item $\mathcal{G}$ seems undefined. How is this different from $\mathbb{R}^d$? I believe we are permitting the feasible set of $\bbtheta$ to be unbounded within $\mathbb{R}^d$, correct?
%%
%\item $ \bar{\tau}_{0,a} (\epsilon) >K$ needs to be defined here, as does the set of local minima/maxima, and all the quantities in Theorem \ref{Theorem:Exit_time}. For instance, the definition of $M,d^+,K$ are missing rigorous/specific definitions. Some of that is defined at the beginning of Appendix \ref{Proof:exittime}, but it needs to be here instead/also.
%%
%\item The statement formalizing the transition probabilities of the limiting process is missing from this section (specifically, the contents of Appendix \ref{apx_transition_time}.
%%
%\end{enumerate}
%%
%}
\begin{theorem}(Exit Time Dependence on Tail Index) \label{Theorem:Exit_time}
%
%
Under Assumptions \ref{Assum:Q0}- \ref{assmp:domaing}, if the value function $J$  is initialized near a local maxima $\bar{\bbtheta}_i$, then the policy gradient update in \eqref{eq:policy_gradient_iteration00} under a heavy-tailed parameterization with tail index $\alpha$ associated with its induced stochastic error \eqref{eqn:SGD_L}, the likelihood of exit time being more than $K$ is upper bounded as 
% from the neighborhood  of $\bar{\bbtheta}_i$  at an exit time  $\bar{\tau}_{0,a}$  
%with a positive probability given by 
%
\begin{align}\label{eq:exit_time_theorem}
%
\!\!\! \mathcal{P}^{\bbtheta_0} \!\left(  \bar{\tau}_{0,a} (\epsilon) >\!K\right) 
 %
  &\leq \frac{2}{\epsilon^{\rho \alpha}} \epsilon^{\alpha} (d^+)^{-\alpha}   \!+\!   \mathcal{O} \bigg( \!\! \left({d} K \eta^{2-(1/\alpha)}\right)^{\beta}  \!\!\! \nonumber \\ & + \mathcal{O} \! \left(1- \left(1-C_{\alpha}d^{1+\frac{\alpha}{2}}\eta \exp{(\alpha M_J\eta)}\epsilon^{\alpha}\left(\frac{\xi}{3}\right)^{-\alpha} \right)^{K} +\delta   \right)  
 %
\end{align}
 
%
%\red{AB: what is $k_1$ here?}
where, $\bbtheta_0$ is the point of initialization, $d^+$  denotes distance  between $\bbtheta_0$ and the boundary of $\mathcal{G}$,  $\rho$ is a positive constant such that $\rho \in (0,1)$,  $\alpha$  the  tail-index,  $d$ is the dimension of $\bbtheta$. Moreover, the H\"{o}lder continuity constant satisfies $\beta \in (0,\alpha-1)$, $\delta >0$,  $\xi>0$,  $\eta$ is the step-size, $k_1$ is a function of stepsize $\eta$, $k_1: = 1/\eta^{\alpha-1}$, and $\epsilon$ is the coefficient multiplying the jump process.
%\red{AB: In Mert's paper, along with the expression in \eqref{eq:exit_time_theorem}, they have an additional expression which talks about the exit time in expectation. That expression is much more clean and is intuitive. Can we have a similar expression here? For instance, for the SGD setting, the average exit time is given by 
%%
%\begin{align}
%	\EE[\bar{\tau}_{0,a}]= \frac{\alpha}{2}\frac{a^\alpha}{\epsilon^\alpha}(1+\mathcal{O}(\epsilon^\delta)).
%\end{align}
%%
%From the above expression, it is very clear that the average exist time is proportional to the width of the region given by $a$. So for a fixed $\alpha$, the exist time would be higher for a larger width region. In a similar manner, for a fixed width region, the average exit time would be less for higher $\alpha$ due to the present of $\epsilon^{\alpha}$ term in the denominator because $\epsilon\rightarrow 0$. We need something like this discussion. I think presenting this average exit time makes more sense in the table than the probabilistic expression.   }
\end{theorem}
%
See proof in Appendix \ref{Proof:exittime}. Let us take a closer look at the result in the above Theorem. In \eqref{eq:exit_time_theorem}, the left hand side denotes the probability of an event that the exit time (minimum number of iterations to exit the local maxima) is strictly greater than $K$. Note that intuitively, we need to show that the probability of this event is as low as possible which implies that the algorithms exits the local maximum within $K$ number of iterations with high probability. So, for the  right hand side of \eqref{eq:exit_time_theorem}, the lower is better. It is interesting to note that with  small noise limit ($\epsilon \to 0$) of  \eqref{eq:exit_time_theorem},   the likelihood in the right hand side of \eqref{eq:exit_time_theorem} depends  on the  distance of $\bbtheta_0$ from the boundary $\partial \mathcal{G}$ and tail-index, $\alpha$. Further  the probability of escape from local extrema is inversely proportional to the width of the boundary.  Therefore, the proposed heavy-tailed setting prefers wide maxima and  its escape probability increases  with  heavier  tail indices. In order to get better intuition of the results with respect to conventional policy gradient approach, we summarize the  corresponding average exit time results for the single dimensional case in the Table \ref{table_1}. Note that since there exists only a single direction of exit for one dimensional case, this results coincide with the expressions discussed in  \cite{imkeller2006first,nguyen2019first}. In contrast to proposed heavy-tailed setting wherein exit time is a function of width of the  neighborhood, exit time for vanilla PG (cf. Table \ref{table_1})  depends exponentially on the  function value at the extremas. 
%
\begin{theorem} (Transition Time Dependence on Tail Index)\label{theorem: transitiontym}
Suppose Assumptions \ref{Assum:Q0}- \ref{assmp:domaing} hold and the value function $J$  is initialized near a local maxima $\bar{\bbtheta}_i$. Then in the limit $\epsilon \to 0$,  the policy gradient update in \eqref{eq:policy_gradient_iteration} under a heavy-tailed parameterization with tail index $\alpha$ associated with its induced stochastic error \eqref{eqn:SGD_L}, transitions from $\mathcal{G}_i$ to the boundary of $(i+1)$-th local maxima with a probability, $\mathcal{P}^{\bbtheta_0}( \bbtheta^{k} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) $  lower bounded by the following function of the tail index $\alpha$:
%
 \begin{align} \label{eqn:thm4}
%
\lim_{\epsilon \to 0} \mathcal{P}^{\bbtheta_0}( \bbtheta_{k\eta} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) \geq \frac{d_{ij}^{-\alpha}}{((d_{ij}^+)^{-\alpha} + (-d_{ij}^-)^{-\alpha}}  - \delta,
%
\end{align}
where $\delta >0$ and distance function $d_{ij}^+(\bbtheta)\!:=\! \inf \{ t\! >\!0\!:\! g_{{i}_{\bbtheta}}(t) \!\in\! \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1} \!\}$ and $d_{ij}^-(\bbtheta)\!:=\! \sup \{ t \!<\!0\!:\! g_{{i}_{\bbtheta}}(t) \!\in\! \Omega_i^- (\bar{\delta}) \cap \partial \mathcal{G}_{i+1} \!\}$. 
%
\end{theorem}
% \textcolor{green}{need to more rigorously define $\lambda_k^\alpha$ and $N$. Also, what is $\xi$? This is a positive constant but why is it defined? To introduce slack in a neighborhood of $a$? Moreover, $p_i^{-}$ seems unused in \eqref{eq:exit_time_theorem}. Why is it defined?}

%$U_R$, $\gamma$ are the parameters of proposed RL setting, positive constants, $C, \, C_1\, C_2$,   are functions of dissipativity constants of score function, 
%\begin{align}
%\mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq &  \exp{\left(-K\eta \epsilon^{\alpha} \frac{1}{a^{\alpha}\alpha}(1+C\epsilon^{\delta})\right)} (1+ C \epsilon^{\delta}) +  \exp{(M\eta)}  M \eta  \frac{   C_1  \left( 1 + C_2 \left(\frac{U_R}{(1-\gamma)^2}  (m +b)/2   + C \frac{d}{k_1^{1/\alpha}}   \right)K\eta \right)^{\beta}}{\xi/3}     \nonumber \\
% & +  1- \left(1-C_{\alpha}d^{1+\frac{\alpha}{2}}\eta \exp{(\alpha M\eta)}\epsilon^{\alpha}\left(\frac{\xi}{3}\right)^{-\alpha}\right)^{K} +\delta,
%%\end{align}
%\begin{proof}
%The proof is provided 
%\end{proof}

See proof in Appendix \ref{sec:proofthm4}. Similar to the exit time results, the transition time probability is a function of the width of boundary and the tail index.   The  corresponding expressions in a single dimensional case  for both vanilla policy gradient and proposed approach are summarized in Table \ref{table_1}.  Transition times are asymptotically exponentially distributed in the limit of small noise and scales like $1/\epsilon^{\alpha}$.  On the other hand, transition time for Brownian is exponential distributed with  $\epsilon^\alpha$ replaced by $e^{2 J(\cdot)/\epsilon^2}$.  This means that in the small noise
limit, Brownian-motion driven policy search needs exponential time to transit to another
minimum whereas Levy-driven gradient descent dynamics need only polynomial time and highlights the better exit guarantees with heavier tail index. 
%\green{we need a comment about how the transition time only depends on the width of the peak, but not the height, in contrast to classical (fat-tailed) central limit theorem associated with Gaussians. Classical result like \cite{raginsky2017non} should also have some exponential dependence on the parameter dimension that we are alleviating, right?}
%
%\begin{center}
%	\begin{tabularx}{01\textwidth} { 
%  | >{\centering\arraybackslash}X 
%  | >{\raggedright\arraybackslash}X | >{\raggedright\arraybackslash}X|}
%		\hline
%Algorithm  & Exit time & Transition time   \\
%		\hline
%	HPG &  $ \mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq \frac{2}{\epsilon^{\rho \alpha}} \epsilon^{\alpha} (d^+)^{-\alpha}  + \mathcal{O} \left( \frac{d}{k_1^{1/\alpha}} K \eta\right)^{\beta}  + \mathcal{O} \left(d^{1+\frac{\alpha}{2}} \epsilon^{\alpha}\left(\frac{\xi}{3}\right)^{-\alpha}\right)^{K} $  &  $\lim_{\epsilon \to 0} \mathcal{P}^{\bbtheta_0}( \bbtheta_{k\eta} \in \Omega_i^+ (\bar{\delta}) \cap \partial \mathcal{G}_{i+1}) \geq \frac{d_{ij}^{-\alpha}}{((d_{ij}^+)^{-\alpha} + (-d_{ij}^-)^{-\alpha}}  - \delta$\\
%  		\hline
%  	Vanilla PG &  $\mathcal{P}^{\bbtheta_0} \left(  \bar{\tau}_{0,a} (\epsilon) >K\right) 
% \leq $ \blue{Need to find this expression: immediate step} &  \\
%
%		\hline
%	\end{tabularx}
%	%\caption{First Exit time of Algorithms}
%\end{center}
%\blue{Note: Once we finalize the analysis for the above Theorem we can directly invoke results for Vanilla PG with constant variance. We need to the exit time for Brownian in  $\mathbb{R}^d$ from the literature and relate it to discrete process. Note that the Theorems from Mert et al. is for one dimensional case. Below, I briefly summarize the corresponding expression of SDE for Brownian case. This would be our starting point and we follow same steps as followed for the above Theorem except that L\'{e}vy process will now be replaced by Brownian. Also, lot of parts will be simplified as we just need Lipschitz continuity. }\green{please fill in this table as it pertains to usual policy parameterizations (e.g., Gaussian)}

